Simplicity in Complexity : Explaining Visual Complexity using Deep Segmentation Models

The complexity of visual stimuli plays an important role in many cognitive phenomena, including attention, engagement, memorability, time perception and aesthetic evaluation. Despite its importance, complexity is poorly understood and ironically, previous models of image complexity have been quite complex. There have been many attempts to find handcrafted features that explain complexity, but these features are usually dataset specific, and hence fail to generalise. On the other hand, more recent work has employed deep neural networks to predict complexity, but these models remain difficult to interpret, and do not guide a theoretical understanding of the problem. Here we propose to model complexity using segment-based representations of images. We use state-of-the-art segmentation models, SAM and FC-CLIP, to quantify the number of segments at multiple granularities, and the number of classes in an image respectively. We find that complexity is well-explained by a simple linear model with these two features across six diverse image-sets of naturalistic scene and art images. This suggests that the complexity of images can be surprisingly simple.

==> main_old.tex <==
% % --------------------------------------------------------------------------



% % Annual Cognitive Science Conference
% % Sample LaTeX Paper -- Proceedings Format
% % 

% % Original : Ashwin Ram (ashwin@cc.gatech.edu)       04/01/1994
% % Modified : Johanna Moore (jmoore@cs.pitt.edu)      03/17/1995
% % Modified : David Noelle (noelle@ucsd.edu)          03/15/1996
% % Modified : Pat Langley (langley@cs.stanford.edu)   01/26/1997
% % Latex2e corrections by Ramin Charles Nakisa        01/28/1997 
% % Modified : Tina Eliassi-Rad (eliassi@cs.wisc.edu)  01/31/1998
% % Modified : Trisha Yannuzzi (trisha@ircs.upenn.edu) 12/28/1999 (in process)
% % Modified : Mary Ellen Foster (M.E.Foster@ed.ac.uk) 12/11/2000
% % Modified : Ken Forbus                              01/23/2004
% % Modified : Eli M. Silk (esilk@pitt.edu)            05/24/2005
% % Modified : Niels Taatgen (taatgen@cmu.edu)         10/24/2006
% % Modified : David Noelle (dnoelle@ucmerced.edu)     11/19/2014
% % Modified : Roger Levy (rplevy@mit.edu)     12/31/2018

% %% Change "letterpaper" in the following line to "a4paper" if you must.

% \documentclass[10pt,letterpaper]{article}

% \usepackage{cogsci}
% \usepackage[textsize = tiny,backgroundcolor=blue!10!white]{todonotes}
% \newcommand{\topd}[1]{\todo{#1}}

% \cogscifinalcopy % Uncomment this line for the final submission 
% \usepackage{graphicx}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{xcolor}
% \usepackage{placeins}
% \usepackage{amsmath}
% \usepackage{dirtytalk}
% \usepackage{pslatex}
% \usepackage{apacite}
% \usepackage[symbol]{footmisc}
% \usepackage{float} % Roger Levy added this and changed figure/table
%                    % placement to [H] for conformity to Word template,
%                    % though floating tables and figures to top is
%                    % still generally recommended!

% %\usepackage[none]{hyphenat} % Sometimes it can be useful to turn off
% %hyphenation for purposes such as spell checking of the resulting
% %PDF.  Uncomment this block to turn off hyphenation.

% %\setlength\titlebox{4.5cm}
% % You can expand the titlebox if you need extra space
% % to show all the authors. Please do not make the titlebox
% % smaller than 4.5cm (the original size).
% %%If you do, we reserve the right to require you to change it back in
% %%the camera-ready version, which could interfere with the timely
% %%appearance of your paper in the Proceedings.


% \title{Simplicity in Complexity}

% \author{{\large \bf Kevin Shen$^{1,*}$, Surabhi S Nath$^{1,2,3,*}$, Aenne Brielmann$^{2}$, Peter Dayan$^{1,2}$} \\
%   $^1$Max Planck Institute for Biological Cybernetics, Tübingen, Germany \\
%   $^2$University of Tübingen, Tübingen, Germany \\
%   $^3$Max Planck School of Cognition, Leipzig, Germany
%   }

% \begin{document}

% \maketitle
% \footnotetext{* indicates equal contribution}

% \begin{abstract}

% The complexity of visual stimuli plays an important role in many cognitive phenomena, including attention, engagement, memorability, time perception and aesthetic evaluation. Despite its importance, complexity is poorly understood and ironically, previous models of image complexity have been quite \textit{complex}. There have been many attempts to find handcrafted features that explain complexity, but these features are usually dataset specific, and hence fail to generalise. On the other hand, more recent work has employed deep neural networks to predict complexity, but these models remain difficult to interpret, and do not guide a theoretical understanding of the problem. Here we propose to model complexity using segment-based representations of images. We use state-of-the-art segmentation models, SAM and FC-CLIP, to quantify the number of segments at multiple granularities, and the number of classes in an image respectively. We find that complexity is well-explained by a simple linear model with these two features across six diverse image-sets of naturalistic scene and art images. This suggests that the complexity of images can be surprisingly simple.
% % and show its potency at capturing complexity across various datasets and domains.

% % There have been a many attempts at modelling  human perception of complexity in natural images. These works either use handcrafted features, which often fail to generalise or employ deep neural networks, which are hard to interpret.
% % We adopt a middle ground, leveraging the power of state-of-the-art segmentation models to arrive at the core components of complexity. Using SAM and FC-CLIP, we quantify the number of segments in an image at multiple granularities, including named segments. We show that a simple linear regression model comprising of two features excellently explains complexity across six image-sets. Ironically we find that a model of complexity can be surprisingly simple!

% \textbf{Keywords:} 
% visual complexity; natural images; image segmentation; foundation models
% \end{abstract}

% \section*{Introduction}

% The subjective complexity of sensory stimuli plays an important role in many cognitive phenomena, including attention, engagement, memorability, time perception or aesthetic evaluation \cite{kyle2023complexity, palumbo2014examining, sun2021curious, van2020order}, and is relevant to a wide range of real-world applications such as advertising, web design, and computer graphics \cite{king2020influence, pieters2010stopping, ramanarayanan2008dimensionality, reinecke2013predicting, wu2016complexity}. It is therefore important to understand the factors and mechanisms underlying the perception of complexity. Most empirical and theoretical work concerns artificial or
% naturalistic images \cite{chikhman2012complexity, gartus2017predicting, guo2023image, machado2015computerized, nagle2020predicting, nath2023relating}; the
% latter are the focus of our work.

% There is by now a range of datasets containing human ratings of the
% complexity of various sub-categories of naturalistic images---we consider
% \textit{RSIVL} (\textit{RSIVL-RS1}) \cite{corchs2016predicting}, \textit{VISC} (\textit{VISC-C}) \cite{kyle2023characterising}, \textit{Savoias} \cite{saraee2020visual} and \textit{IC9600} \cite{feng2022ic9600}. Duly, there has then been a number of
% attempts to predict these ratings, and thereby understand the
% computations concerned. Note, though, that these methods have hitherto largely been applied on their own, separate, datasets, rather than being directly compared. The methods fall into two broad categories: using either simple (often linear) combinations of handcrafted image features, or  modern convolutional neural networks (CNNs) as predictors or feature extractors. We advocate a middle ground, revealing an unexpected degree of simplicity in modelling complexity.

% For the first category of methods, several qualitative and quantitative image features have been proposed and shown to predict complexity. These include the number and variety of elements, colour, edge density, file size, Fourier slope, HOG and information-theoretic measures such as entropy and information gain \cite{van2020order}. Corchs \textit{et al.}  compiled 11 measures based on spatial, frequency and color properties which were combined linearly to fit perceived complexity ratings on the \textit{RSIVL} dataset. They found the number
% of regions, frequency factor and number of colours received the largest weights \cite{corchs2016predicting}.

% Equally, Kyle-Davidson \textit{et al.} proposed measures of clutter (see also \cite{fan2017visual, olivia2004identifying, rosenholtz2007measuring}),
% entropy and patch-wise symmetry as determinants of complexity, showing good performance on the \textit{VISC} dataset.

% The advantage of hand-crafted features is that they are largely interpretable. However, they are often dataset-specific, possibly due to the difficulty of evaluating such rather subjectively-defined measures in general. Perhaps as a result, a large number of these potentially noisy features seem to be required to predict subjective complexity well.

% More recently, it has become popular to exploit the computational capabilities of deep neural networks to extract relevant image features. Analysis on \textit{Savoias} dataset, comprising of 1400 images across 7 categories showed that activations from intermediate layers of a CNN pretrained on object or scene recognition correlated best with human complexity ratings \cite{saraee2020visual}. These authors also compared unsupervised and supervised methods, suggesting that supervision can improve prediction.

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/complexity_model_copy.pdf}
%     \caption{
%     Overview of methods. Our complexity model is shown. Images from across 8 different scenes and art image-sets are passed through 2 segmentation models--SAM, for segmentation, and FC-CLIP for semantic segmentation. Example images are shown for 4 image-sets, namely \textit{RSIVL}, 
%     \textit{IC9600 scenes},
%     \textit{IC9600 paintings} and \textit{Savoias Supremantism} (\textit{Sav. Sup.}).
%     The outputs of SAM are shown as Segmented Images, where the detected segments are highlighted, and the outputs of FC-CLIP are shown as Semantic Image Classes where the image with detected classes and a list of classes obtained are shown. For clarity, only a subset of classes detected by FC-CLIP are shown in each image. The predicted segments and class-instances from SAM and FC-CLIP are counted and the counts are deemed \textit{num\_seg} and \textit{num\_class}. These two features are then transformed using square root function. The resulting $\sqrt{num\_seg}$ and $\sqrt{num\_class}$ features are linearly combined to estimate complexity.
%     }
%     \label{fig:pipeline}
% \end{figure*}

% Feng and colleagues built further on this work, first by introducing a large-scale visual complexity dataset comprising on 9600 images across 8 semantic categories, and then providing a CNN-based method predicting scores and activation maps \cite{feng2022ic9600}. This model achieved high test performance, outperforming previous methods.

% However, although such CNN-based models perform well, and can even generalise competently to unseen images, they are hard to interpret (as activation maps do not convey much information, and can also be unreliable \cite{bilodeau2024impossibility}) and do not guide a theoretical understanding of the problem.

% Here, we benefit from both categories of methods. We use modern foundation models \cite{bommasani2021opportunities} to evaluate particular hand-crafted features in a way that
% generalizes across many classes of images. We then combine these features linearly to predict complexity.

% To choose hand-crafted features, we start from the observation that features that fragment images in meaningful ways tend to estimate complexity relatively well (for example, clutter in
% \cite{kyle2023characterising} or the number of regions in
% \cite{corchs2016predicting}). We therefore leverage the capabilities of state of the art (SOTA) image segmentation models to extract relevant segments from the image at multiple spatial granularities. Such models are the closest existing approximations to how humans represent scenes for two main reasons: first, the models are trained using a vast amount of annotations from several humans and hence reflect relevant inductive biases, and second, the architecture of CNNs and transformers are inspired by the human visual processing systems and generalize surprisingly well to unseen images. With the help of such models, we obtain semantically consistent segments at different spatial granularities relevant to perceptual image processing \cite{epstein2019scene}. We then derive from them the core components of perceived complexity.

% With improved quality of feature extraction and evaluation, we make the central observation that only few features are necessary to predict complexity well, justifying the claim that complexity can be surprisingly simple.

% % \section{Introduction}

% % How do people perceive complexity in the world? Human perception of complexity has been a frequently researched topic. Reasons for this interest is that complexity is known to drive several other cognitive phenomenon such as attention, engagement, memorability, time perception or aesthetic evaluation \cite{kyle2023complexity, sun2021curious, van2020order, palumbo2014examining}, and is relevant to a wide range of real-world applications such as advertising, web design, and computer graphics \cite{}. As a result, it is important to understand the factors and mechanisms underlying the perception of complexity. Owing to the ready availability of generation techniques and richly annotated data, a common modality for the study of complexity is the visual domain, using both artificial \cite{gauvrit2014natural, nath2023relating, ciocca2015complexity, chikhman2012complexity} and naturalistic images, the latter being the focus of our work.

% % Several attempts have been made to arrive at a model of complexity for naturalistic images. However, the definitions and realisations of complexity vary largely across studies. 
% % % \textcolor{red}{(can provide examples if required)}. 
% % Within these works, two major streams are identified---the first, using handcrafted image features as predictors of perceived complexity, and the second, using convolutional neural networks (CNNs) as predictors or feature extractors. We discuss both these streams along with their costs and benefits, and motivate our method as a useful middle ground.

% % With respect to the first stream of work, several qualitative and quantitative image features have been proposed and shown to be indicative of perceived complexity. These include the number and variety of elements, colour, edge density, file size, Fourier slope, HOG and information-theoretic measures such as entropy and information gain \cite{van2020order}. Kyle-Davidson \textit{et al.} proposed measures of clutter (see also \cite{olivia2004identifying, rosenholtz2007measuring, fan2017visual}), entropy and patch-wise symmetry as determinants of complexity in the \textit{VISC-C} dataset. Corchs \textit{et al.} compiled 11 measures based on spatial, frequency and color properties which were linearly combined to fit perceived complexity ratings on the \textit{RSIVL} dataset. They found the number of regions, frequency factor and number of colours received the largest weights \cite{corchs2016predicting}. 
% % % \textcolor{red}{Can add another ref here if required}.  
% % % Alongside low-level image features, they also suggested the role of high-level semantic content, proposing a ``dual information" framework of complexity perception \cite{kyle2023characterising}.
% % While such models are convenient to build, and are highly interpretable, the features are handcrafted and often dataset-specific.

% % % https://journals.plos.org/plosone/article?id=10.1371/journal.pone.0207879
% % % Art - gif compression - https://bpspsychub.onlinelibrary.wiley.com/doi/full/10.1348/000712610X498958
% % % VISC low level - low-level image features and high-level semantic content
% % % Identifying the Perceptual Dimensions of Visual Complexity of Scenes 
% % % https://www.sciencedirect.com/science/article/pii/S0924271622000545?casa_token=4E2R7LUuAKsAAAAA:IokpT8DfZAuB60oaDAPp1-cPfPpynOTjIqc12gsuWuEp-AtF3_BBojxtwe8Tto51-4NZHar6PA
% % % Information theory - An Information Theory Framework for the Analysis of Scene Complexity - https://onlinelibrary.wiley.com/doi/abs/10.1111/1467-8659.00331
% % % Nadal
% % % In scenes and paintings - https://journals.plos.org/plosone/article/file?id=10.1371/journal.pone.0072412&type=printable
% % % https://journals.plos.org/plosone/article/file?id=10.1371/journal.pone.0072412&type=printable

% % Subsequently, the second stream of studies emerged, utilizing the computational capabilities of deep neural networks to extract relevant image features. 
% % % Work by Kyle-Davidson \textit{et al.} was extended to employ a neural network for predicting complexity \cite{kyle2022predicting}. They reported that the neural network performance was boosted when the low-level features were integrated, suggesting the roles of both low-level and high-level image features. 
% % % Nagle and Lavie showed that a CNN with weights pre-trained on an object recognition task predicted complexity ratings superior to a model using low-level features \cite{nagle2020predicting}. 
% % Analysis on \textit{Savoias} dataset, comprising of 1400 images across 7 categories showed that activations from intermediate layers of a CNN correlated the most with human complexity ratings \cite{saraee2020visual}. They also compared unsupervised and supervised methods suggesting that supervision can improve prediction. Feng \textit{et al.} built further on this work, first by introducing a large-scale visual complexity dataset comprising on 9600 images across 8 semantic categories, followed by providing a CNN-based method predicting scores and complexity maps using weak-supervision \cite{feng2022ic9600}. This model achieved high test performance, outperforming previous methods. Although such models yield relatively good performance which may generalise well to unseen images, they are hard to interpret (activation maps do not convey much information and can also be unreliable \cite{bilodeau2024impossibility}) and are not guided by a theoretical understanding of the problem.

% % NN - Predicting human complexity perception of real-world scenes,  
% % VISC NN - low-level image features and high-level semantic content - https://ieeexplore.ieee.org/abstract/document/9897953/authors#authors
% % Savoias -  Elham Saraee, Mona Jalal, and Margrit Betke, “Visual
% % complexity analysis using deep intermediate-layer features,” Computer Vision and Image Understanding, vol.
% % 195, pp. 102949, 2020.
% % IC9600 - 

% % In this work, we tackle the mentioned limitations in both streams, and delineate the core components of complexity by adopting a middle-ground. There is evidence that features that fragment the image in meaningful ways tend to estimate complexity relatively well (for example, clutter in \cite{kyle2023characterising} or the number of regions in \cite{corchs2016predicting}). However, not many studies employed such measures, perhaps due to the lack of methods to extract meaningful fragments. In this regard, we hypothesize that the reason for the failure of these handcrafted features is likely not the inqdequency of the measure itself but the inqdequency of methods for computing the measures sufficiently well. The quantitative ways in which such features are extracted from naturalistic images are non-standard, purely image-driven and hence may be far from how humans derive them. For this, we leverage the capabilities of state of the art (SOTA) image segmentation models to extract relevant segments from the image at multiple spatial granularities. Such models are the closest existing approximations to how humans represent scenes for two main reasons: first, the models are trained using a vast amount of annotations from several humans and hence reflect relevant inductive biases, and second, the architecture of CNNs are inspired by the human visual system enabling generation to unseen images. With the help of such models, we obtain semantically consistent segments at different spatial granularities relevant to perceptual image processing \cite{epstein2019scene}. We then derive from them the core components of perceived complexity. With improved quality of image features, we also achieve model simplicity, a key contribution of our work.

% % % middle ground since intermediate complexity features work best
% % % ref: https://www.nature.com/articles/nn870
% % % object-features - https://www.sciencedirect.com/science/article/pii/S1071581920301257?casa_token=c5QwNcAaTIMAAAAA:3StBa00OPoRd1OaB5vLGTLF-jy0bbXvsjrqnWrmpRrKkPRvi_ZoSJuVpVfaddWZNDx3cn-eQIQ#sec0015

% \section{Method}

% We develop a parsimonious model of the perceived complexity of naturalistic images using two types of segmented features, namely the number of segments, and the number of named classes, extracted from SOTA segmentation models. Our method is described in Figure \ref{fig:pipeline}. We also use an additional measure called patch-symmetry
% (borrowed from \cite{kyle2023characterising}) to address a main failure mode of our model.


% \subsection{Datasets}

% We use 4 freely available naturalistic image datasets with corresponding subjective complexity ratings, namely \textit{RSIVL} \cite{corchs2016predicting}, containing 49 scene images; \textit{VISC} \cite{kyle2023characterising}, containing 800 scene images across 12 sub-categories, \textit{Savoias} \cite{saraee2020visual}, containing 1400 images across 7 categories, and \textit{IC9600}, containing 9600 images across 8 categories \cite{feng2022ic9600}. We use the mean subjective complexity per image across raters (there were between 10 to 26 raters per image across datasets) as  ground truth. We restrict to scenes and art image categories and omit advertisement (\textit{Savoias} and \textit{IC9600}) and visualisation (\textit{Savoias}) categories since they contain substantial amounts of text. We combine similar image categories within a dataset to generate 8 image-sets for analysis: (1) \textit{RSIVL}, containing all \textit{RSIVL-RS1} images; (2) \textit{Savoias Scenes} (\textit{Sav. Scenes}), comprising of \textit{Savoias} scene and object categories; (3) \textit{IC9600 Scenes} (\textit{IC9. Scenes}), comprising of \textit{IC9600} scene, object, person, transportation and architecture categories; (4) \textit{Savoias Art} (\textit{Sav. Art}); (5) \textit{Savoias Suprematism} (\textit{Sav. Suprematism}); (6) \textit{IC9600 Paintings} (\textit{IC9. Paintings}); (7) \textit{VISC}, containing all \textit{VISC-C} images, and lastly (8) \textit{Savoias Interior Design} (\textit{Sav. Int}), which is considered separately as it contains software-generated 3D-rendered images.

% %Images in each image-set are passed through two segmentation models, SAM and FC-CLIP where respectively multi-granularity segments and higher-level object classes are extracted.

% % We apply minimal data pre-processing and use mean complexity ratings from each dataset as-is. We investigate our model using two image categories: naturalistic scenes and art. We use three naturalistic datasets: RSIVL \cite{}, Savoias Scenes and Objects (a combination of the Savoias Scenes and Objects datasets), and IC9600 Scenes (a combination of the Object, Scenes, Architecture, Person and Transportation images from the IC9600 dataset). We also use three art datasets: Savoias Art, Savoias Suprematism, and IC9600 Paintings.

% % \begin{table*}[th]
% %     \centering
% %     \begin{tabular}{c|c|c|c|c}
% %         \hline
% %          Dataset & Number of Images & Categories & Method of Annotation & Baseline model \\ \hline
         
% %          \textit{RSIVL RS1}& 49 & Scenes & & 11 handcrafted features\\
% %          \textit{VISC-C} & 800 & Scenes & & 4 handcrafted features, CNNs\\
% %         \textit{Savoias} & 1400 & Scenes, Objects & & Unsupervised and supervised CNNs\\
% %          \hline
% %     \end{tabular}
% %     \caption{Summary of Datasets}
% %     \label{tab:my_label}
% % \end{table*}

% \subsection{Finding Segments using a Foundational Segmentation Model}

% We extracted segments in images using the SOTA Segment Anything Model (SAM) \cite{kirillov2023segment}. SAM detects blobs of segments in an image at different scales. SAM was trained on the largest public segmentation dataset to date, is capable of zero-shot generalization, and achieves SOTA performance. Based on pilot studies, we set the spatial granularity parameter \textit{points-per-side} to $64$. This allowed the network to find finer segments, and correlated well with ground truth complexity. We set all other parameters of SAM to their default values and evaluated the total number of detected segments per image (\textit{num\_seg}). 

% \subsection{Finding Classes using Open-vocabulary Semantic Segmentation}

% We found the nameable class instances in an image using FC-CLIP \cite{yu2023convolutions}. FC-CLIP is an open-vocabulary panoptic segmentation algorithm that can find multiple instances of each class, and achieves SOTA performance \cite{yu2023convolutions}. We use panoptic semantic segmentation to predict classes because multi-scale methods like Semantic SAM \cite{chen2023semantic} produced many false positives. We set all parameters of FC-CLIP to default and evaluated the number of detected classes per image (\textit{num\_class}).

% Intuitively, FC-CLIP finds the most salient, lower granularity semantic classes in the image while SAM finds sub-components of these classes at higher granularities. As a result, \textit{num\_seg} is larger than \textit{num\_class} for all images. 

% \begin{table*}[h]
% \begin{center} 
% \caption{Model performance on 6 image-sets and comparison with previous models. The models from previous work are classified as being based on either handcrafted features, or Convolutional Neural Networks (CNNs). * for supervised methods indicate their own \textit{test} set. Bold indicates the best model.} 
% \label{tab:mainresults} 
% \begin{tabular}{lcccccc} 
% \hline
% \hline
% Model/Image-set & \textit{RSIVL} & \textit{Sav. Scenes} & \textit{IC9. Scenes} & \textit{Sav. Art} & \textit{Sav. Suprematism} & \textit{IC9. Paintings} \\
% \hline
% \textbf{Handcrafted features} \\
% \hline
% \quad Corchs 1 (10 features) & 0.66	& 0.62 & 0.70 & 0.68 & 0.80 & 0.53 \\
% \quad Corchs 2 (3 features) & 0.77 & - & - & - & - & -\\
% \quad Kyle-Davidson 1 (2 features) & 0.68 & 0.54 & 0.54 & 0.55 & 0.79 & 0.49 \\
% \hline
% \textbf{CNNs} \\
% \hline
% \quad Saraee (transfer) & 0.72 &	0.67 &	0.59 &	0.55 &	0.72 &	0.58 \\
% \quad Kyle-Davidson 2 (supervised) & 0.50 & 0.36 &	0.41 &	0.30 &	0.15 &	0.33 \\
% \quad Feng (supervised) & 0.83 &	\textbf{0.79} &	\textbf{0.94*} & \textbf{0.81} &	0.84 &	\textbf{0.93*} \\
% \hline
% \textbf{Our method} \\
% \hline
% \quad $\sqrt{\textit{num\_seg}}$ & 0.78 &	0.65 &	0.81 &	0.67 &	0.89 &	0.82 \\ 
% \quad $\sqrt{\textit{num\_class}}$ & 0.70 &	0.75 &	0.73 &	0.56 &	0.27 &	0.67 \\ 
% \quad $\sqrt{\textit{num\_seg}} + \sqrt{\textit{num\_class}}$ & \textbf{0.83} &	0.78 &	0.84 &	0.73 &	\textbf{0.89} &	0.83 \\ 
% \hline
% \hline
% \end{tabular} 
% \end{center} 
% \end{table*}

% \begin{figure*}[h]
%   \centering
%   \captionsetup[subfigure]{labelformat=empty,font=scriptsize}

%   % Adding Column Titles
%   \begin{tabular}{p{0.14\textwidth}p{0.14\textwidth}p{0.15\textwidth}p{0.14\textwidth}p{0.15\textwidth}p{0.15\textwidth}}
%     \centering\textbf{\textit{RSIVL}} & \centering\textbf{\textit{Sav. Scenes}} & \centering\textbf{\textit{IC9. Scenes}} & 
%     \centering\textbf{\textit{Sav. Art}} & \centering\textbf{\textit{Sav. Suprematism}} & \centering\textbf{\textit{IC9. Paintings}} \tabularnewline
%     \end{tabular}

%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/rsivl_high.jpg}
%     \caption{G: 89 (100),
%              P: 86 (100),\\
%              S: 449 (100),
%              C: 18 (80)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savsce_high.jpg}
%     \caption{G: 89 (99),
%              P: 110 (100),\\
%              S: 467 (100),
%              C: 66 (100)}

%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/ic9scene_high.jpg}
%     \caption{G: 100 (100),
%              P: 96 (100),\\
%              S: 571 (100),
%              C: 67 (100)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savart_high.jpg}
%     \caption{G: 100 (100),
%              P: 101 (100),\\
%              S: 276 (100),
%              C: 30 (100)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savsup_high.jpg}
%     \caption{G: 100 (100),
%              P: 104 (100),\\
%              S: 119 (100),
%              C: 4 (84)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/ic9paint_high.jpg}
%     \caption{G: 84 (100),
%              P: 88 (100),\\
%              S: 420 (100),
%              C: 32 (98)}
%   \end{subfigure}

%   \vspace{2mm}

%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/rsivl_low.jpg}
%     \caption{G: 7 (0),
%              P: 13 (0),\\
%              S: 2 (0),
%              C: 2 (8)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savsce_low.jpg}
%     \caption{G: 10 (3),
%              P: 10 (0),\\
%              S: 50 (11),
%              C: 0 (0)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/ic9scene_low.jpg}
%     \caption{G: 24 (1),
%              P: 26 (0),\\
%              S: 11 (0),
%              C: 0 (0)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savart_low.jpg}
%     \caption{G: 0 (0),
%              P: 12 (0),\\
%              S: 23 (9),
%              C: 0 (0)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/savsup_low.jpg}
%     \caption{G: 3 (7),
%              P: -15 (0),\\
%              S: 1 (0),
%              C: 1 (0)}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.16\textwidth}
%     \includegraphics[width=\linewidth,height=\linewidth]{figures/examples/ic9paint_low.jpg}
%     \caption{G: 4 (0),
%              P: 22 (0),\\
%              S: 4 (0),
%              C: 2 (4)}
%   \end{subfigure}
%   \caption{Images with the highest (top row) and lowest (bottom row) complexity predictions for the 6 image-sets in Table \ref{tab:mainresults}. G = ground truth complexity from 0 to 100, P = predicted complexity, S = $\textit{num\_seg}$, C = $\textit{num\_class}$. Percentiles of the corresponding values are shown in brackets. The highest predicted images have many entities and hence high \textit{num\_seg} and \textit{num\_class}. The lowest predicted images have only a few entities and hence low \textit{num\_seg} and sometimes zero \textit{num\_class}.}
%   \label{fig:examples}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/ic9600_heatmap.png}
%     \caption{Mean and standard deviation of the ground truth subjective complexity in different bins of $\sqrt{\textit{num\_seg}}$ and $\sqrt{\textit{num\_class}}$ for \textit{IC9600 Scenes}. 
%     % Means show that complexity increases with $\sqrt{\textit{num\_seg}}$ and $\sqrt{\textit{num\_class}}$. 
%     % Standard deviations reveal that FC-CLIP might over- or under-predict classes.
%     }
%     \label{fig:model_heatmap}
% \end{figure}

% \subsection{Linear Regression Model}

% We estimate subjective complexity using multiple linear regression. A preliminary examination showed that subjective complexity scales roughly linearly with $\sqrt{num\_seg}$ and $\sqrt{num\_class}$, hence, we apply a square-root transformation to our features. We used the \texttt{statsmodels} OLS function in Python to fit our models.
% % correlation, Spearman correlation, $R^2$, adjusted $R^2$, Akaike information criterion (AIC) and Bayesian information criterion (BIC). 
% We perform 3-fold cross-validation $M$ times, where $M$ is larger for smaller datasets, and report the average Spearman correlation over all \textit{test} sets. We compare our models to six baselines from previous work. These baselines include three handcrafted feature-based baselines---two from \cite{corchs2016predicting}--Corchs 1, comprising of their 3 best features M8, M5 and M10 (only tested on RSIVL since we were unable to implement M8 (\textit{number of regions}) to apply it for other datasets), Corchs 2 comprising of 10 features M1 to M11 (excluding M8) and one baseline from \cite{kyle2023characterising} comprising of their clutter and patch-wise symmetry measures. The other three are CNN baselines, namely the supervised method from \cite{kyle2023characterising}, the transfer-learning method from \cite{saraee2020visual} and the supervised method from \cite{feng2022ic9600}.

% % Along with reporting the variance explained by our model for comparison with the other models, we evaluate the mean and standard deviation of our model in discrete bins of $\sqrt{num\_seg}$ and $\sqrt{num\_class}$, as the separate components of the error. 

% % We compare the variance our model explains to previous results reported for each dataset, as well as baselines using statistical features (entropy, symmetry, ?). See \ref{Appendix:baselines} for details about these features. ). For the RSIVL and VISC datasets, we also report the \say{one-vs-rest} noise-ceiling because we have participant-level ratings. The one-vs-rest noise-ceiling is computed by treating the ratings of a single participant as the independent variable and the mean rating of all other participants as the dependent variable. It is also a measure of the participant's \say{typicality}. Although not a strict upperbound, the one-vs-rest noise-ceiling is determined by individual differences in complexity judgments which limits the amount of variance any mechanistic model can plausibly explain.  We also report the \say{half-versus-half} noise-ceiling in the Appendix \ref{Appendix:noise-ceiling}.

% \section{Results}

% \subsection{Excellent performance on natural scenes and art}

% Table \ref{tab:mainresults} shows the performance of our models and baselines for 6 image-sets. We see that our linear model with $\sqrt{\textit{num\_seg}}$ and $\sqrt{\textit{num\_class}}$ attains a Spearman correlation between 0.73 to 0.89 with human complexity judgments across natural scenes and art image-sets. Notably, our model performs better than all handcrafted feature baselines, the transfer-learning neural network method from \cite{saraee2020visual} and the supervised neural network from \cite{kyle2023characterising}. 

% It performs similarly to the supervised neural network from \cite{feng2022ic9600}. The exceptions are the test datasets from the same paper and \textit{Savoias Art}. This neural network \textit{directly} learns a high-dimensional mapping from image to complexity, thereby discovering features that best predict complexity in a supervised way. We show that in many cases, this high-dimensional relationship can be distilled down to simply the number of segments and named instances in the image. Hence, we provide evidence that complexity is computable from segmentation features, rather than requiring features that are explicitly optimized for complexity. 
% % This is consistent with the view that complexity judgment is a metacognitive process \cite{} which has evidence in neuroscience \cite{}.

% We also compared the full model with versions restricted to just one of the $\sqrt{\textit{num\_seg}}$ or $\sqrt{\textit{num\_class}}$ terms. We see that both terms contribute to the variance explained for all datasets except \textit{Savoias Suprematism}, where $\sqrt{\textit{num\_class}}$ fails to explain additional variance on top of $\sqrt{\textit{num\_seg}}$. This is because \textit{Savoias Suprematism} contains abstract art images with geometric shapes, and FC-CLIP fails to find appropriate nameable classes as in its training set. However, for \textit{Savoias Suprematism}, the model with only $\sqrt{\textit{num\_seg}}$ already explains high variance and achieves performance superior to all other models, suggesting that the number of segments at multiple granularities drives perceived complexity in images composed of geometrical shapes that lack overt semantics (at least for art-novice raters). 

% Figure \ref{fig:examples} shows the images with the highest and lowest predicted complexity from each of the 6 image-sets in Table \ref{tab:mainresults}. The highest predicted images are those with many entities and hence high $\sqrt{\textit{num\_seg}}$ and $\sqrt{\textit{num\_class}}$. The lowest predicted images have only a few entities and hence low $\sqrt{\textit{num\_seg}}$ and sometimes zero $\sqrt{\textit{num\_class}}$.

% Figure \ref{fig:model_heatmap} shows the mean and standard deviation of the ground truth subjective complexity 
% % (Figure \ref{fig:heatmap_gt}), and predicted complexity (Figure \ref{fig:heatmap_pred}) 
% for images for each bin of $\sqrt{\textit{num\_seg}}$ and $\sqrt{\textit{num\_class}}$ on an example image-set, \textit{IC9600 Scenes}. In general, and as expected, mean ground truth complexity increases with increasing $\sqrt{\textit{num\_class}}$ and increasing $\sqrt{\textit{num\_seg}}$ (also well-matched to predictions) showing that a complex image is one with both a large number of segments and classes.
% The standard deviation of the subjective complexity, which contributes markedly to the prediction error, is particularly high in the bins with the greatest and least $\sqrt{\textit{num\_class}}$. This suggests that FC-CLIP might over- or under-predict classes. The largest discrepancies lie in the bin with the highest $\sqrt{\textit{num\_seg}}$ and the lowest $\sqrt{\textit{num\_class}}$. Here, FC-CLIP often fails to find any nameable segments at all. 
% % On the other hand, as expected, the variance in each bin for predicted complexity is nearly 0 as they map to similar \textit{num\_seg} and \textit{num\_class} values.

% \subsection{Failure mode: symmetry and structure}
% \label{sec:symm}


% \begin{figure*}
%     \centering
%     \begin{minipage}{0.62\linewidth}
%         \centering
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth]{figures/examples/sav_59_orig.jpg}
%             \caption{G: 16,
%                      P: 56, 
%                      Symm: 97}
%           \end{subfigure}
%           \hfill
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth]{figures/examples/sav_59_sam.png}
%             \caption{$\textit{num\_seg}$: 204 (78.5)}
%           \end{subfigure}
%           \hfill
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth]{figures/examples/59.jpeg}
%             \caption{$\textit{num\_class}$: 37 (87)}
%           \end{subfigure}
        
%           \vspace{0.1cm}
        
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth,height=2.5cm]{figures/examples/visc_orig.jpg}
%             \caption{G: 56,
%                      P: 83, 
%                      Symm: 53}
%           \end{subfigure}
%           \hfill
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth,height=2.5cm]{figures/examples/visc_sam.png}
%             \caption{$\textit{num\_seg}$: 538 (100)}
%           \end{subfigure}
%           \hfill
%           \begin{subfigure}{0.327\textwidth}
%             \includegraphics[width=\linewidth,height=2.5cm]{figures/examples/visc_fcclip.jpg}
%             \caption{$\textit{num\_class}$: 3 (9.3)}
%           \end{subfigure}
%         \caption{Example image with one of the highest prediction errors from the \textit{VISC} (top row) and \textit{Sav. Int} (bottom row) datasets. From left to right: original image, SAM output, FC-CLIP output. G = ground truth complexity from 0 to 100. P = predicted complexity. Symm = patch-symmetry percentile. Percentiles of \textit{num\_seg} and \textit{num\_class} are also shown in brackets. SAM finds too many segments and without accounting for structure this leads to overprediction. In the top image, FC-CLIP also finds high $\textit{num\_class}$. In the bottom image $\textit{num\_class}$ is low but $\textit{num\_class}$ does not contribute significantly to the regression for \textit{VISC}. However, both images have high patch-symmetry.}
%         \label{fig:examples_fail}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.34\linewidth}
%         \centering
%         \includegraphics[width=\linewidth,height=5.9cm]{figures/savint_symm_error.png}
%         \caption{The relationship between patch-symmetry and prediction error for \textit{Sav. Int.} Model overprediction (indicated by positive prediction error) occurs when patch-symmetry is high. Linear
%         regression reveals a significant Pearson correlation of 0.51.}
%         \label{fig:plot_error_symmetry}
%     \end{minipage}
%     % \caption{Overall Caption}
% \end{figure*}

% The statistics of segments and classes at multiple granularities explain most of the variance in the datasets we tested. However, the structure in the image, \textit{i.e.}, the spatial and functional relationships between elements is also known to be an important contributor to complexity (\cite{chipman1977complexity, ichikawa1985quantitative}, Gestalt theory of perception). Indeed, we find that segment statistics alone are not enough to adequately explain complexity judgments in two other image-sets: \textit{VISC} and \textit{Savoias Interior Design}. Figure \ref{fig:examples_fail} shows an example from each dataset with the highest prediction errors. In each case, our model over-predicts complexity because SAM finds too many segments without accounting for the fact that many segments are arranged in a spatial pattern (books in the top row and windows in the bottom row). Further, \textit{num\_class} does not contribute to reducing complexity in such cases, either because it is also high (since the uniqueness of classes is not accounted for), or because the weight of the \textit{num\_class} term is learned to be low (for example in \textit{VISC}) We see that both of these images have high patch-symmetry (defined in \cite{kyle2023characterising}). Figure \ref{fig:plot_error_symmetry} illustrates a significant, positive correlation between patch-symmetry and model error (prediction minus ground truth), showing that our model tends to over-predict when the image is more spatially symmetric, \textit{i.e.} has more spatial structure. Table \ref{tab:visc_int_results} shows that when \textit{patch\_symmetry} is added as a feature to the regression, our model improves in Spearman correlation by atleast 0.12, and becomes competitive with most baselines.
% % However, the performance still falls short of \cite{feng2022ic9600} and Corchs 1 on Sav. Int showing that there's room to improve on the feature our model uses to capture the variance in the structure. 
% % better than most baselines and competitive with the \cite{feng2022ic9600} supervised neural network.


% \begin{table}[h]
% \begin{center} 
% \caption{Model performance on \textit{VISC} and \textit{Savoias Interior Design} (\textit{Sav. Int}) datasets with and without the \textit{patch\_symmetry} feature, and comparison with previous models. Bold indicates the best model.} 
% \label{tab:visc_int_results} 
% \vskip 0.12in
% \begin{tabular}{lcc} 
% \hline
% \hline

% Model/Image-set & \textit{VISC} & \textit{Sav. Int} \\
% \hline
% \textbf{Handcrafted features} \\
% \hline
% \quad Corchs 1 (10 features) & 0.62 &	0.85 \\
% \quad Kyle-Davidson 1 (2 features) & 0.60 &	0.74 \\
% \hline
% \textbf{Neural network} \\
% \hline
% \quad Saraee (transfer) & 0.58 &	0.75 \\
% \quad Kyle-Davidson 2 (supervised) & - &	0.56 \\
% \quad Feng (supervised) & \textbf{0.72} &	\textbf{0.89} \\
% \hline
% \textbf{Our method} \\
% \hline
% \quad $\sqrt{\textit{num\_seg}} + \sqrt{\textit{num\_class}}$ & 0.56 &	0.61 \\ 
% \quad $\sqrt{\textit{num\_seg}} + \sqrt{\textit{num\_class}} + \textit{patch\_symm}$ & 0.68 &	0.80 \\ 
% \hline
% \hline
% \end{tabular} 
% \end{center} 
% \end{table}


% \section{Discussion}

% We presented a linear model of complexity using two features extracted using SOTA segmentation neural networks: $\textit{num\_seg}$ and $\textit{num\_class}$. Our model outperforms most baselines achieving a Spearman correlation between 0.73 to 0.89 with subjective complexity ratings across six tested image-sets of naturalistic scenes and art. As a result, our model provides a simple explanation of perceived complexity that generalizes across multiple domains and image types. Our results suggest that segment-based representations are good proxies for the cognitive processes underlying human judgments of complexity, a result that could be extended to attention, memorability, aesthetic evaluation, etc.

% Our model performs better than all handcrafted feature-based baselines. A possible reason for this is that \textit{num\_seg} is a significant improvement over previously suggested features for image fragmentation (such as \say{number of regions} from \cite{corchs2016predicting}) that approximate the segments in an image. Further, to our best knowledge, we are the first to exploit named-segments corresponding to semantic classes to predict complexity, whose count provides an estimate of the number of lower granularity segments in an image.
% % The  \textit{num\_class} feature provides a novel way of estimating the variety of entities/objects in an image.

% Importantly, the segments and classes are both computed by neural networks trained on large datasets of human annotations. Therefore, the predictions are likely to be semantically meaningful, reflecting not only pixel information but also the annotator's prior experiences with the contents of the images in the training set. The annotations and hence segments also encompass multiple levels of spatial and semantic granularity, capturing contributions to complexity across scales. 
% This is in contrast to past works that have tried to approximate spatial granularity and semantic variety using only sliding windows or pyramid scaling of filters \cite{corchs2016predicting, guo2023image, kyle2022predicting, kyle2023characterising}.

% % From the perspective of an agent that acts in the world given visual input, the complexity of visual stimuli is related to the amount of useful information to the agent for taking actions which is related to the number of objects and hence segments (it feels like we can point to some body of literature here, the connection must have been made, Tankred's paper comes to mind, also the Aaronson paper on "useful information" as complexity but maybe also resource rationality, the connection to "objects" explicitly is less clear) \cite{}. That is to say, objects and segments are more fundamental and previously tried image-wide features such as entropy, and colorfulness. Many image-wide features are likely trying to approximate the number of named and unnamed segments. After all, an image with many segments tends to be colorful, have a lot of edges, and be entropic. 

% % Previous works have hypothesized the contribution of named, symbolic entities to perceived complexity \cite{} but we are the first to empirically show this in that $\text{num\_class}$ added to the variance explained of all 6 datasets we tested. 
% % In \cite{kyle2023characterising}, the neural network is interpreted to provide "high-level" information to complement the "low-level information" provided by features. "High-level" information is present in both the named segments and the unnamed segments that are detected because the annotators are likely using both bottom-up and top-down information to annotate segments \cite{}.
% Our model performance was generally comparable to the supervised neural network of \cite{feng2022ic9600}, which was trained on a large dataset to directly predict complexity. The difference in performance can be explained by the fact that the neural network potentially utilizes many more than two features and conditionally chooses those features based on the context and distribution of images. However, we have shown that only two features can explain complexity equally well on multiple datasets and domains, elucidating a simpler view of complexity. 
% % Further, for datasets like \textit{RSIVL}, where both models achieve similar high performance ($0.83$ Spearman correlation), it is likely that no further variance in subjective complexity could plausibly be explained, owing to the inherent rating noise and individual differences.

% % It is plausible that \cite{feng2022ic9600} outperforms our model on \textit{Sav. Art} because the neural network potentially utilizes many more than two features and conditionally chooses those features based on the context and distribution of images. 

% In addition, unlike the CNN models, our model is highly interpretable. As we demonstrate in Figure \ref{fig:examples_fail}, we can attribute predictions or diagnose failure cases by visually inspecting the outputs of SAM and FC-CLIP. Also, the contributions of the segments and classes to the complexity score can be clearly elucidated (as the square root of their counts).

% % Another benefit of our model is interpretability. I think here we mean with our model you can visually inspect the segments predicted by SAM and infer failure cases - for example we could tell there was a problem with SAM overpredicting segments without accounting for structure. I don't think you can do something analgous, as effectively with previous methods. The attention maps from the supervised NNs aren't very informative
% % suggesting the possibility that these neural networks are principally using a segmentation approach to predicting complexity. 
% % (Do we say something about the attention maps of the neural network methods and how they relate to areas with a lot of segments)? In fact, the neural network baseline from \cite{saraee2020visual} is trained on object recognition. Therefore, their method can be seen as an approximate way to pool/add/count the number of object and object component/features in the image.
% % Our method ourperforms many of the CNN baselines, such as the \cite{saraee2020visual} and \cite{kyle2022predicting}. Furthermore, our method is more interpretable than pure CNN-based methods, as we can effectively visualise the outputs of SAM and FC-CLIP and use them to compute relevant image attributes (such as counts of segments and classes).
% % - How num\_class is a new feature never implemented this way in the past.
% % - low-level high-level combined importance point has been made in VISC, relate to that
% % - how $\text{num\_seg}$ is different from earlier implementations of num\_objects and better (how it encompasses variance from a lot of other bottom up features)
% % 
% % \subsection{Limitations}

% However, our model has limitations. The accuracy of our model depends on the accuracy of the segments and classes predicted by SAM and FC-CLIP. Currently, SAM is incapable of detecting thin, \say{one-dimensional} patterns.
% % There could be false-positives and missed segments (for example, SAM missed segments when the image contained only 1D patterns). 
% FC-CLIP sometimes misses salient classes or repeated classes (failing to predict \textit{any} classes for some images outside its training distribution, \textit{e.g.} images in \textit{Sav. Suprematism}) and doesn't predict nested classes at multiple granularities (\textit{e.g.} both the ``house" and its ``window"). As the SOTA segmentation models improve, we expect the performance and interpretability of our model to also increase further.

% We also addressed the inability of $\textit{num\_seg}$ and $\textit{num\_class}$ to account for structure in an image which reduces perceived complexity. We saw that adding \textit{patch-symmetry} to the regression led to competitive performance on \textit{VISC} and \textit{Sav. Int} image-sets. However, as part of future works, we aim to build a more parsimonious model using a segment-based feature of structure. For example, scene-graphs \cite{chang2021comprehensive} or generative programs \cite{sable2022language} can be used to organize the named entities detected by FC-CLIP by their spatial and semantic relationships, and image complexity can be derived from the complexity of these representations, for example as their compressibility \cite{dehaene2022symbols, karjus2023compression, mahon2023minimum}.
% % Further, our method only evaluates the number of classes, disregarding the correctness of the classes, hence the errors of the FC-CLIP model  cascade to our regression model. 
% % The interpretability of our model also depends on the segments that are predicted. False-positives and negatives make the number of segments difficult to understand. Overall, as segmentation models become better, we expect our method to explain more of the variance in complexity ratings and become more interpretable.

% % - failure related points:
% % - failure modes directly improvable by improving the segmentation models themselves.
% % - how interpretable is our model really (features themselves are but SAM and FC-CLIP are not)
% % - Also how we don't care about the accuracy of the segments and classes, only the count and it's impact 


% % \subsection{Experts, amount of time given to judge complexity}

% % Construed more broadly, the complexity of images depends also on the perceiver. This is most obvious in art, especially abstract art. Where experts can find paintings very complex but novices find the same paintings to be low complexity. (Do we want to relate this to the notion of useful information for the perceiver/agent? This also links to the idea of generative graph and program encoding "useful information" in the next section). All datasets we tested, the complexity ratings were given by novices. This is most apparently for the Savoias Suprematism dataset where the images are abstract art and complexity is almost entirely explained by the number of segments - which probably wouldn't be true if experts were judging the images. The complexity ratings were also judged by participants were who given very little time. The fast perception of an image and its complexity may differ greatly from the slow perception of an image (there's currently no datasets for this). (For example when art experts judge a piece, they're doing slow perception). This needs to tested in future experiments. Not only the complexity ratings but the segment annotations (both segment and classes) themselves are also provided by non-experts (MTurkers?). It is likely that experts would "see fundamentally different objects, elements, patterns and components" in an image compared to a novice. However, what this work shows is that there is a set of universal primitive/segments that work well to explain complexity in a lot of naturalistic images and art.

% % \subsection{Intra, inter-group differences}
% We modeled subjective complexity ratings which was the mean rating across multiple raters. However, complexity judgments are known to vary across both individuals or groups (age, cultures, etc.) \cite{gartus2017predicting}. For the art datasets, the complexity ratings were given by art-novices and would likely differ significantly from ratings of art-experts \cite{bimler2019art, pihko2011experiencing}. These individual differences could be caused by differences in the segments people perceive (the regions of an image they consider to be part of the same segment). For example, different individuals may segment at different granularities. Individual differences can also be caused by the mapping from the perceived segments to complexity. Explicitly accounting for individual variability using subject-specific data (for example by fine-tuning the regression or segmentation models) will be an important part of future work.
% % In either case, the model (SAM, FC-CLIP, or the linear regression weights) could potentially be fine-tuned to each individual to accommodate their differences \cite{NN-fine-tuning-paper}.
% % Both in the perceived segments, since we only have a single segmentation model that isn't catered to a particular person to their complexity judgments.
% % Not only the complexity ratings but the segment annotations (both segment and classes) themselves are also provided by non-experts (MTurkers?).
% % Accomodate these differences, fine-tuning. Segmentation scales. Complexity function as function of segments could change as well

% % While there is intergroup variability in perceived complexity, for example between experts and novices, there is also likely intragroup variability. From preliminary investigations, we saw substantial variation in the complexity ratings in the \textit{RSIVL} and \textit{VISC} datasets.

% % The complexity ratings were also judged by participants were who given very little time. The fast perception of an image and its complexity may differ greatly from the slow perception of an image (there's currently no datasets for this).

% % \subsection{Future Works implementing Structure (Scene Graphs, Generative Programs)}


% In conclusion, we develop a parsimonious and interpretable account of human perceived complexity in naturalistic images using segmentation-based methods, showing that complexity can be surprisingly simple given the right image representations.

% % In conclusion, our work developed a simple and interpretable account of human-perceived complexity in naturalistic images using segmentation-based methods. We emphasize the take home message that complexity can be surprisingly simple!
% % This result urges other researchers to experiment with segment-based representations to better understand other related cognitive phenomena.

% % Such representations can provide a unifying view of the features we presented in this paper, capturing the distribution of types of entities/objects and heir spatial and functional relationships to each other as well as their number. 
% % The LOT literature proposes that complexity is related to the shortest program, and in this case the shortest program in the human language-of-thought that encodes all the useful information in the stimuli. Can potentially provide unifying explanation. Future works can explicitly examine the role of spatial and functional relationship between objects and how they impact complexity. And whether the LOT framework can accurately predict complexity.

% % - Individual Differences, where the complexity ratings came from (non-experts vs experts), how reliable is the mean rating?
% % - expert vs non expert labelers
% % - amount of time it takes the annotators to rate and how they could be a different perceptive process
% % - Where the segments of the models (and class predictions) come from (Turk raters) and how this relates to their experience and long-term memory -- \textcolor{red}{this point is sort of included already in the intro}

% % \subsection{Other modalities}

% % Our method relies on the existence of entities, segments. But this begs the question what a segment is in other domains such as audio, or language. What is the complexity of a musical piece or song? What is the complexity of a paragraph, an essay, or a book? (Cite some previous works that have discussed this). While the complexity of all these modalities are very different, they all seem to share some notion of segments at different levels in a granularity of abstraction. And complexity depends on the segments at every level. (For example in a book there's the theme, there's the sentence structure, and then there's the vocabulary which can be simple or challenging). Similar idea for music, there are notes and there are bars, rifts, chorus, etc. (Here we can speculate how the complexity may also scale with the number of elements in a fixed size of the stimuli, for example a fixed number of pages in a book, or a duration of music).

% % \section{Acknowledgments}

% % In the \textbf{initial submission}, please \textbf{do not include
% %   acknowledgements}, to preserve anonymity.  In the \textbf{final submission},
% % place acknowledgments (including funding information) in a section \textbf{at
% % the end of the paper}.

% % \nocite{ChalnickBillman1988a}
% % \nocite{Feigenbaum1963a}
% % \nocite{Hill1983a}
% % \nocite{OhlssonLangley1985a}
% % % \nocite{Lewis1978a}
% % \nocite{Matlock2001}
% % \nocite{NewellSimon1972a}
% % \nocite{ShragerLangley1990a}


% \bibliographystyle{apacite}

% \setlength{\bibleftmargin}{.125in}
% \setlength{\bibindent}{-\bibleftmargin}

% \bibliography{CogSci_Template}


% \end{document}
